Towards Cross-speaker Reading Style Transfer on Audiobook Dataset

Cross-speaker style transfer aims to extract the speech style of the given reference speech, which can be reproduced in the timbre of arbitrary target speakers. Existing methods on this topic have explored utilizing utterance-level style labels to perform style transfer via either global or local scale style representations. However, audiobook datasets are typically characterized by both the local prosody and global genre, and are rarely accompanied by utterance-level style labels. Thus, properly transferring the reading style across different speakers remains a challenging task. This paper aims to introduce a chunk-wise multi-scale cross-speaker style model to capture both the global genre and the local prosody in audiobook speeches. Moreover, by disentangling speaker timbre and style with the proposed switchable adversarial classifiers, the extracted reading style is made adaptable to the timbre of different speakers. Experiment results confirm that the model manages to transfer a given reading style to new target speakers. With the support of local prosody and global genre type predictor, the potentiality of the proposed method in multi-speaker audiobook generation is further revealed.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> tex/grammer.tex <==
\section{Experiments}
\label{sec:expr}
\subsection{Datasets and model details}
\label{ssec:expr:dataset_model}
We evaluate the proposed cross-speaker reading style transfer method on the following
disjoint datasets:

\textbf{MST-Originbeat}: A neutral Mandarin corpus offered by the ICASSP 2021 M2VOC challenge \cite{9414001},
with one female and one male speaker,
each with 5,000 utterances.


\textbf{DB}: A private neutral Mandarin dataset
with 10,000 utterances from
another female Chinese speaker, named DB6.

\textbf{Audiobook\_FM}: A private Mandarin audiobook dataset with 8 speakers and 2 types of genres:
fairy tale and Chinese martial arts fiction.
A female and a male speakers cover both of the 2 genres,
each of the other 6 speakers only covers one of the 2 genres.
One of the 6 speakers is DB6, who only reads the fairy tale documents.
This dataset has a total amount of 1,315 paragraphs,
which is 13,718 utterances adding up to 24.3 hours.

When applied to the proposed chunk-wise reading style model,
each short paragraph in the Audiobook\_FM dataset is regarded as a chunk,
whose global genre label is assigned based on the topic of the including document:
either \textbf{fairy tale} or \textbf{martial arts fiction}.
While for datasets MST-Originbeat and DB,
each chunk is made up of 10 randomly sampled utterances
that are voiced by the same speaker,
and all chunks share the same global genre label: \textbf{neutral}.

In our experiment,
the model is trained 380k steps for the first stage,
%[lixiangv0]
260k steps for the second stage.
All classifiers are trained by cross entropy loss with weight set as $0.05$.
A pre-trained HiFi-GAN \cite{DBLP:conf/nips/KongKB20} vocoder
is utilized to generate audio.

\subsection{Cross-speaker reading style transfer}
\label{ssec:expr:style_trans}

Based on the proposed model,
we aim to transfer the reading style of
fairy tale and martial arts fiction to neutral speakers in MST-Originbeat,
or speakers in whose training data the target reading style is absent.
Given the target speaker identity and the audios of reference paragraph with target reading style,
this could be achieved by combining:
(i) the averaged speaker timbre GSE vector
over all chunks in the training data of the target speaker;
(ii) the global genre GSE vector and LPE sequences
extracted from the reference audio chunk.
We evaluate the reading style transfer results on the reserved test set,
the proposed synthesized speech keeps local prosody and global genre
close to the reference utterance,
but with the timbre of target speakers.
For audio samples,
please check our demo website\footnote{\scriptsize https://thuhcsi.github.io/is2022-cross-speaker-reading-style-transfer}.

\subsubsection{Baseline}
For comparison, we establish an embedding-table-based baseline method by
replacing the 2 global branches of the multi-scale style model with
a speaker embedding table and a global genre embedding table.
Which is similar to the setting of \cite{xie2021multi},
except that there is an additional embedding table of the global genre
to accommodate the audiobook dataset.

\subsubsection{Evaluation}
We conduct a Mean Opinion Score (MOS) test on 
66 utterances from the test set,
with 26 native Chinese speakers serve as subjects.
Each test group is made up by a synthesized audio $\tilde{M}$,
the ground truth reference audio $M_{ref}$ and the target speaker audio $M_{tgt}$,
The subjects are asked to rate $\tilde{M}$
on a scale of 1 to 5 regrading 3 different aspects:
(i) its style similarity to $M_{ref}$;
(ii) its timbre similarity to $M_{tgt}$;
(iii) its audio quality.
As shown in Table.\ref{tab:mos},
the proposed model beats baseline model on
all evaluation scores,
which verifies the effectiveness
of the proposed chunk-wise multi-scale cross-speaker style model
in enhancing cross-speaker reading style transfer performance.


In addition to the subjective timbre similarity test,
we use a pre-trained speaker verification (SV) model to 
extract speaker embedding vectors from the synthesized audios and the target speaker audios.
The objective evaluation of speaker timbre similarity of each synthesized speech is thus obtained
by computing the cosine similarity between the extracted vector
and the averaged vectors of the corresponding target speaker.
As shown in Table.\ref{tab:mos},
the overall outcomes are generally consistent with subjective timbre similarity test results.

\subsection{Ablation study}
\label{ssec:expr:abl}
We conduct 3 settings of ablation experiments to reveal the functionality of each component of the proposed method.

(i) We remove the global genre branch in the style model,
leaving the timbre branch as the only global module.
As shown in the subjective test results,
there is noticeable style similarity degradation
in the transferred speech of the ablating model,
which indicates the necessity of explicitly modeling
the global genre in reading style transfer.
In the meantime, 
the timbre similarity scores are observed to be improved,
since on the global scale, the ablating model is focused on speaker timbre only.

(ii) We replace the chunk-wise GSE extracting method
with an ordinary utterance-wise approach.
The style similarity evaluation results are downgraded
due to the shrunken receptive field of the global scale modules.
After visualizing the extracted GSE vectors via t-SNE,
the genre GSE vectors of the fairy tales are found to be confused
with those of the martial arts fiction
(right column of the 2nd row in Figure.\ref{fig:t-sne}).
On the other hand,
considering there are unique GSE vectors for each utterance,
more information is conveyed
to help the model converge better,
which explains the slight promotion in audio quality.

% \subsubsection{Switchable adversarial classifiers}
(iii) We employ vanilla adversarial classifiers
to disentangle GSE vectors of different branches,
instead of the proposed switchable adversarial classifiers (SAC).
As revealed in Table.\ref{tab:mos},
the speaker timbre similarity of transferred speeches
drops significantly.
Furthermore, in the t-SNE plot of the extracted timbre GSE vectors,
the samples of $<\mathrm{SPKER1\_fiction}>$ and $<\mathrm{SPKER1\_fairy\ tale}>$
end up in different clusters
(left column of the 3rd row in Fig.\ref{fig:t-sne}),
which confirms there is still considerable genre information
entangled in the timbre GSE vector.
These details support that the proposed SAC is crucial for
timbre and style disentanglement on disjoint dataset scenarios.

\subsection{Automatic audiobook generation}
Based on the proposed cross-speaker reading style transfer model,
an automatic audiobook generation system could be constructed
by incorporating a text analysis model
which predicts the LPE and genre from given book content.
In our practice,
the prediction model is implemented with RNN and linear layers,
which takes BERT \cite{devlin2018bert} token embedding and Tacotron-2 phoneme embedding as its inputs,
similar to existing methods \cite{hodari2021camp,xie2021multi}.
According to the predicted genre label and the identity of the desired speaker,
the GSE vectors on each branch could be obtained
by choosing the averaged GSE vectors over the training data of the target genre/speaker.
Together with the predicted LPE and text sequence,
the speeches of the target speaker reading the material with the predicted style
is eventually generated.
The inference results are presented on our demo site.

\label{ssec:expr:abl}

==> tex/x_format.tex <==

\section{Page layout and style}

Authors should observe the following rules for page layout. A highly recommended way to meet these requirements is to use a given template (Microsoft Word\textregistered\ or \LaTeX) and check details against the corresponding example PDF file. Given templates, Microsoft Word\textregistered\ or \LaTeX, can be adapted/imported easily in other software such as LibreOffice, Apple Pages, Lua\LaTeX, and Xe\LaTeX, but please be careful to match the layout of the provided PDF example.

\subsection{Basic layout features}

\begin{itemize}
\item Proceedings will be printed in DIN A4 format. Authors must submit their papers in DIN A4 format.
\item Two columns are used except for the title section and for large figures that may need a full page width.
\item Left and right margin are 20 mm each. 
\item Column width is 80 mm. 
\item Spacing between columns is 10 mm.
\item Top margin is 25 mm (except for the first page which is 30 mm to the title top).
\item Bottom margin is 35 mm.
\item Text height (without headers and footers) is maximum 235 mm.
\item Headers and footers must be left empty.
\item Check indentations and spacings by comparing to this example file (in PDF).
\end{itemize}

\subsubsection{Headings}

Section headings are centered in boldface with the first word capitalized and the rest of the heading in lower case. Sub- headings appear like major headings, except they start at the left margin in the column. Sub-sub-headings appear like sub-headings, except they are in italics and not boldface. See the examples in this file. No more than 3 levels of headings should be used.

\subsection{Text font}

Times or Times Roman font is used for the main text. Font size in the main text must be 9 points, and in the References section 8 points. Other font types may be used if needed for special purposes. It is VERY IMPORTANT that while making the final PDF file, you embed all used fonts! To embed the fonts, you may use the following instructions:
\begin{enumerate}
\item For Windows users, the bullzip printer can convert any PDF to have embedded and subsetted fonts.
\item For Linux/Mac users, you may use \\
   pdftops file.pdf\\
   pstopdf -dPDFSETTINGS=/prepress file.pdf
\end{enumerate}

\LaTeX users: users should use Adobe Type 1 fonts such as Times or Times Roman. These are used automatically by the INTERSPEECH2022.sty style file. Authors must not use Type 3 (bitmap) fonts.

\subsection{Figures}

All figures must be centered on the column (or page, if the figure spans both columns). Figure captions should follow each figure and have the format given in Figure~\ref{fig:speech_production}.

Figures should be preferably line drawings. If they contain gray levels or colors, they should be checked to print well on a high-quality non-color laser printer.

Graphics (i.\,e., illustrations, figures) must not use stipple fill patterns because they will not reproduce properly in Adobe PDF. Please use only SOLID FILL COLORS.

Figures which span 2 columns (i.\,e., occupy full page width) must be placed at the top or bottom of the page.

\subsection{Tables}

An example of a table is shown in Table~\ref{tab:example}. The caption text must be above the table.

\begin{table}[th]
  \caption{This is an example of a table}
  \label{tab:example}
  \centering
  \begin{tabular}{ r@{}l  r }
    \toprule
    \multicolumn{2}{c}{\textbf{Ratio}} & 
                                         \multicolumn{1}{c}{\textbf{Decibels}} \\
    \midrule
    $1$                       & $/10$ & $-20$~~~             \\
    $1$                       & $/1$  & $0$~~~               \\
    $2$                       & $/1$  & $\approx 6$~~~       \\
    $3.16$                    & $/1$  & $10$~~~              \\
    $10$                      & $/1$  & $20$~~~              \\
    $100$                     & $/1$  & $40$~~~              \\
    $1000$                    & $/1$  & $60$~~~              \\
    \bottomrule
  \end{tabular}
  
\end{table}

\subsection{Equations}

Equations should be placed on separate lines and numbered. Examples of equations are given below. Particularly,
% 
\begin{equation}
  x(t) = s(f_\omega(t))
  \label{eq1}
\end{equation}
% 
where \(f_\omega(t)\) is a special warping function
% 
\begin{equation}
  f_\omega(t) = \frac{1}{2 \pi j} \oint_C 
  \frac{\nu^{-1k} \mathrm{d} \nu}
  {(1-\beta\nu^{-1})(\nu^{-1}-\beta)}
  \label{eq2}
\end{equation}
% 
A residue theorem states that
% 
\begin{equation}
  \oint_C F(z)\,\mathrm{d}z = 2 \pi j \sum_k \mathrm{Res}[F(z),p_k]
  \label{eq3}
\end{equation}
% 
Applying (\ref{eq3}) to (\ref{eq1}), it is straightforward to see that
% 
\begin{equation}
  1 + 1 = \pi
  \label{eq4}
\end{equation}

Finally we have proven the secret theorem of all speech sciences. No more math is needed to show how useful the result is!

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figure.pdf}
  \caption{Schematic diagram of speech production.}
  \label{fig:speech_production}
\end{figure}

\subsection{Information for Word users only}

For ease of formatting, please use the styles listed in Table 2. The styles are defined in this template file and are shown in the order in which they would be used when writing a paper. When the heading styles in Table 2 are used, section numbers are no longer required to be typed in because they will be automatically numbered by Word. Similarly, reference items will be automatically numbered by Word when the ``Reference'' style is used.

\begin{table}[t]
  \caption{Main predefined styles in Word}
  \label{tab:word_styles}
  \centering
  \begin{tabular}{ll}
    \toprule
    \textbf{Style Name}      & \textbf{Entities in a Paper}                \\
    \midrule
    Title                    & Title                                       \\
    Author                   & Author name                                 \\
    Affiliation              & Author affiliation                          \\
    Email                    & Email address                               \\
    AbstractHeading          & Abstract section heading                    \\
    Body Text                & First paragraph in abstract                 \\
    Body Text Next           & Following paragraphs in abstract            \\
    Index                    & Index terms                                 \\
    1. Heading 1             & 1\textsuperscript{st} level section heading \\
    1.1 Heading 2            & 2\textsuperscript{nd} level section heading \\
    1.1.1 Heading 3          & 3\textsuperscript{rd} level section heading \\
    Body Text                & First paragraph in section                  \\
    Body Text Next           & Following paragraphs in section             \\
    Figure Caption           & Figure caption                              \\
    Table Caption            & Table caption                               \\
    Equation                 & Equations                                   \\
    \textbullet\ List Bullet & Bulleted lists                              \\\relax
    [1] Reference            & References                                  \\
    \bottomrule
  \end{tabular}
\end{table}

If your Word document contains equations, you must not save your Word document from ``.docx'' to ``.doc'' because when doing so, Word will convert all equations to images of unacceptably low resolution.

\subsection{Hyperlinks}

For technical reasons, the proceedings editor will strip all active links from the papers during processing. Hyperlinks can be included in your paper, if written in full, e.\,g.\ ``http://www.foo.com/index.html''. The link text must be all black. 
Please make sure that they present no problems in printing to paper.

\subsection{Multimedia files}

The INTERSPEECH organizing committee offers the possibility to submit multimedia files. These files are meant for audio-visual illustrations that cannot be conveyed in text, tables and graphs. Just like you would when including graphics, make sure that you have sufficient author rights to the multimedia materials that you submit for publication. The proceedings media will NOT contain readers or players, so be sure to use widely accepted file formats, such as MPEG, Windows WAVE PCM (.wav) or Windows Media Video (.wmv) using standard codecs.

Your multimedia files must be submitted in a single ZIP file for each separate paper. Within the ZIP file you can use folders and filenames to help organize the multimedia files. In the ZIP file you should include a TEXT or HTML index file which describes the purpose and significance of each multimedia file. From within the manuscript, refer to a multimedia illustration by its filename. Use short file names without blanks for clarity.

The ZIP file you submit will be included as-is in the proceedings media and will be linked to your paper in the navigation interface of the proceedings. Causal Productions (the publisher) and the conference committee will not check or change the contents of your ZIP file.

Users of the proceedings who wish to access your multimedia files will click the link to the ZIP file which will then be opened by the operating system of their computer. Access to the contents of the ZIP file will be governed entirely by the operating system of the user's computer.

\subsection{Page numbering}

Final page numbers will be added later to the document electronically. \emph{Do not make any footers or headers!}


\subsection{References}

The reference format is the standard IEEE one. References should be numbered in order of appearance, for example \cite{Davis80-COP}, \cite{Rabiner89-ATO}, \cite[pp.\ 417--422]{Hastie09-TEO}, and \cite{YourName21-XXX}.

\subsection{Abstract}

The total length of the abstract is limited to 200 words. The abstract included in your paper and the one you enter during web-based submission must be identical. Avoid non-ASCII characters or symbols as they may not display correctly in the abstract book.

\subsection{Author affiliation}

Please list country names as part of the affiliation for each country.

\subsection{Number of authors in the author list}

The maximum number of authors in the author list is twenty. If the number of contributing authors is more than twenty, they should be listed in a footnote or in acknowledgement section, as appropriate.

\subsection{Submitted files}

Authors are requested to submit PDF files of their manuscripts. You can use commercially available tools or for instance http://www.pdfforge.org/products/pdfcreator. The PDF file should comply with the following requirements: (a) there must be no PASSWORD protection on the PDF file at all; (b) all fonts must be embedded; and (c) the file must be text searchable (do CTRL-F and try to find a common word such as ``the''). The proceedings editors (Causal Productions) will contact authors of non-complying files to obtain a replacement. In order not to endanger the preparation of the proceedings, papers for which a replacement is not provided in a timely manner will be withdrawn.
